Exosoul: ethical profiling in the digital world

The development and the spread of increasingly autonomous digital technologies in our society pose new ethical challenges beyond data protection and privacy violation. Users are unprotected in their interactions with digital technologies and at the same time autonomous systems are free to occupy the space of decisions that is prerogative of each human being. In this context the multidisciplinary project Exosoul aims at developing a personalized software exoskeleton which mediates actions in the digital world according to the moral preferences of the user. The exoskeleton relies on the ethical profiling of a user, similar in purpose to the privacy profiling proposed in the literature, but aiming at reflecting and predicting general moral preferences. Our approach is hybrid, first based on the identification of profiles in a top-down manner, and then on the refinement of profiles by a personalized data-driven approach. In this work we report our initial experiment on building such top-down profiles. We consider the correlations between ethics positions (idealism and relativism) personality traits (honesty/humility, conscientiousness, Machiavellianism and narcissism) and worldview (normativism), and then we use a clustering approach to create ethical profiles predictive of user's digital behaviors concerning privacy violation, copy-right infringements, caution and protection. Data were collected by administering a questionnaire to 317 young individuals. In the paper we discuss two clustering solutions, one data-driven and one model-driven, in terms of validity and predictive power of digital behavior.

==> Exosoul.tex <==
\subsection{EXOSOUL}
\begin{comment}

EXOSOUL is an overarching research framework that aims at equipping humans with an automatically generated exoskeleton, i.e. a software shield that protects them and their personal data via the mediation of all interactions with the digital world that would result in unacceptable or morally wrong behaviours according to their ethical and privacy preferences. 
Empowering the users with a personalized exoskeleton will introduce more symmetry of power in the present digital world and will effectively put humans in the center. Exoskeletons development also opens unprecedented business opportunities in the field of societal-friendly applications as happened in the case of open source software, which promoted the principles of free software against the monopoly proprietary software producers. Furthermore, bringing back to the user part of the (digital) control helps to solve liability issues in autonomous systems by readdressing responsibility to users according to their specified ethics. In fact, by means of software exoskeletons on the one hand users will be protected by mediating their interactions with the digital world, and on the other hand they will be responsible of the consequences of theirs (ethical) decisions. 


The EXOSOUL project aims to equip humans with an automatically generated exoskeleton, i.e. a software shield that protects them and their personal data through the mediation of all interactions with the digital world that would result in unacceptable or morally wrong behaviors according to their ethical and privacy preferences.
EXOSOUL research framework is tailored to the user's needs and will help to restore symmetry of power in the current digital environment, therefore placing people at the center of the universe once more. As a with open source software, the development of exoskeletons offers up unprecedented financial potential in the sphere of societal beneficial applications, as was the case with the promotion of the principles of free software against monopolistic proprietary software manufacturers. 
As an added benefit, returning certain aspects of (digital) control to users may assist in resolving liability concerns in autonomous systems by re-assigning responsibility to users in accordance with their stated ethics. As a result, users will be protected by software exoskeletons on the one hand, as they will be able to mediate their interactions with the digital world, and on the other hand, they will be held accountable for the consequences of their (ethical) choices. 
\end{comment}

%\begin{comment}

\begin{figure}[!htp]
    \centering
    \includegraphics[width=1\textwidth]{Figures/2.png}
    \caption{EXOSOUL Ethical Engine Scheme with highlight on the work package related to this research.}
    \label{fig:my_label}
\end{figure}

%\end{comment}


%\includegraphics[scale=0.35]{Figures/1.png}

